Surrogate Models for Optimization of Dynamical Systems

Driven by increased complexity of dynamical systems, the solution of system of differential equations through numerical simulation in optimization problems has become computationally expensive. This paper provides a smart data driven mechanism to construct low dimensional surrogate models. These surrogate models reduce the computational time for solution of the complex optimization problems by using training instances derived from the evaluations of the true objective functions. The surrogate models are constructed using combination of proper orthogonal decomposition and radial basis functions and provides system responses by simple matrix multiplication. Using relative maximum absolute error as the measure of accuracy of approximation, it is shown surrogate models with latin hypercube sampling and spline radial basis functions dominate variable order methods in computational time of optimization, while preserving the accuracy. These surrogate models also show robustness in presence of model non-linearities. Therefore, these computational efficient predictive surrogate models are applicable in various fields, specifically to solve inverse problems and optimal control problems, some examples of which are demonstrated in this paper.

==> abstract.tex <==
\begin{abstract}

Driven by increased scientific knowledge and the complexity of dynamical systems, the solution of system of differential equations in optimization problems has become computationally expensive as it relies heavily on numerical simulations. This paper provides mechanism to construct surrogate models from training instances derived from the available evaluations of the true objective functions. These surrogate models combine proper orthogonal decomposition and radial basis functions to achieve accurate responses of aforementioned complex problems with much less computational demand. Using relative maximum absolute error as the measure of accuracy of approximation, the experimental design with combination of symmetric latin hypercube sampling and cubic spline radial basis functions contributed to most accurate system responses. Furthermore, surrogate approach dominated variable order methods in computational time of optimization, while preserving the accuracy in most of the models. The construction of surrogate model is highly CPU intensive and it sometimes lacks robustness in presence of model non-linearities. However these computationally efficient predictive model have found applications in various fields, specifically to solve inverse problems and optimal control problems, some examples of which are demonstrated in this paper.

\end{abstract}
